A Deep Generative Model of Neonatal Cortical Surface Development

The neonatal cortical surface is known to be affected by preterm birth, and the subsequent changes to cortical organisation have been associated with poorer neurodevelopmental outcomes. Deep Generative models have the potential to lead to clinically interpretable models of disease, but developing these on the cortical surface is challenging since established techniques for learning convolutional filters are inappropriate on non-flat topologies. To close this gap, we implement a surface-based CycleGAN using mixture model CNNs (MoNet) to translate sphericalised neonatal cortical surface features (curvature and T1w/T2w cortical myelin) between different stages of cortical maturity. Results show our method is able to reliably predict changes in individual patterns of cortical organisation at later stages of gestation, validated by comparison to longitudinal data; and translate appearance between preterm and term gestation (> 37 weeks gestation), validated through comparison with a trained term/preterm classifier. Simulated differences in cortical maturation are consistent with observations in the literature.

==> junk.tex <==

%We validate our surface-to-surface translation model on the task of modelling cortical development, from sphericalised neonatal cortical surface data. This is a particularly challenging task due to the significant variation in functional and structural organisation of human cortices, even amongst healthy populations, and the rapid and heterogeneous patterns of cortical maturation observed for the developing cortex. Cortical development is known to be affected by preterm birth, although this can be obfuscated by changes during cortical maturation. 

%These factors make the study of developing cortical surfaces a fitting domain for the use of gDL, and gDL models have already been shown to achieve state of the art performance for neurodevelopmental phenotype regression, when benchmarked against classical methods \cite{Fawaz2021.12.01.470730} *amirs, simons, logans segmentation one*.  In this paper, we extend beyond this research to develop two CycleGAN models that model individual changes in cortical maturation and the impact of preterm birth. Such difference maps could act as imaging biomarkers of interest to neonatalogists, since the negative impact of preterm birth on neurodevelopmental outcome remains an area of active research **cite**.

%the first generative model of cortical development to support interpretable predictions of how individual's cortical appearance should change over time or between developmental phenotypes. 

%\section{Related Work}
% \subsection{Image to Image Translation in Cortical Imaging}
% The GAN framework can be adapted for use in a wide variety of generative tasks, and has seen a lot of application to cortical imaging on multiple imaging modalities. GANs are mainly used for image synthesis, and have been applied successfully to T1-weighted MRI images of the brain \cite{j.tom.2018.00042} and brain PET images \cite{islam2020gan,jyoti2020gan}, to generate realistic brain MRIs with tumours \cite{han2018gan,j.tom.2018.00042}, and model brain metastases \cite{10.1145/3357384.3357890} and ageing \cite{xia2021learning}.
% For image-to-image translation, the two most commonly used frameworks are pix2pix \cite{isola2017image} for paired images, and CycleGAN \cite{cyclegan-original} for unpaired images, of which the latter is by far most popular owing to the difficulty in obtaining paired imaging data. Most research has been motivated by cross-modality image generation e.g brain MRI to PET \cite{10.1007/978-3-319-68127-6_2}, MR to CT \cite{9164889} and diffusion-MRI scalar maps from T1-weighted MRI images \cite{gu2019generating} where CycleGANs are used. Pix2pix models mostly find use in denoising \cite{wolterink2017generative,wang20183d} and reconstruction\cite{kim2018improving,chen2018efficient} where the data is inherently paired.
% More recently, GANs have been combined with VAEs to produce more interpretable and controllable models, producing state of the art interpolations of cortical development and degeneration on 2D images and 3D volumes \cite{bass2020icam,bass2021icam,kwon2019generation}.

% \subsection{Geometric Deep Learning}

% % 
% A wide variety of gDL inspired methods have been applied to cortical surface analysis in recent years, from modelling the cortical surface as a graph *cite*, using spatially defined surface convolutions *Cite*, spectral convolutions on the sphere *cite*, to point-cloud based methods *cite amir*. All of these approaches are some compromise between learning powerful expressive filters, having rotational equivariance, and avoiding prohibitively high computational cost. These limitations have been explored in the context of cortical surfaces in a recent benchmarking paper \cite{Fawaz2021.12.01.470730}, where MoNet was found to be a well-performing compromise, with rotational equivariance and good filter power and computational performance.





%%% logans stuff %%%


%\cite{}"identified increased cortical curvature at TEA as a new prognostic biomarker of adverse neurodevelopment in very premature infants." "The most robust predictive model for cognitive score included surface area of the parietal lobe (R), curvature of the temporal lobe (L) and curvature of the posterior cingulate gyrus (L) (table 2). The most robust predictive model for language score included surface area of the parietal lobe (L), curvature of the insula (L) and curvature of the superior temporal gyrus (L)."

%Similar findings in dHCP cohort: "The preterm infants further demonstrated increased curvature measurements compared to the term controls, especially in the mean curvature L2 norm and global curvedness. The right parts of the parietal lobe, posterior medial and inferior temporal gyrus, posterior superior temporal gyrus were significantly higher in the preterm subjects in all the curvature measures." 

%Biological explanation as to why curvature is increased in preterm neonates compared to those born at term: "The cortex of preterm infants at term equivalent PMA has shallower sulci than term infants, as indicated by the smaller sulcal depth values in the present study, and as has been shown by our group and others (Engelhardt et al., 2015; Ramenghi et al., 2007). These shallower sulci retain areas of high curvature at the bottom of sulci and the edges of gyri, but are missing areas of low curvature in the sulcal walls. The effect on curvature-based measures would be to give higher values when averaged over the cortical surface (in the sense of showing greater average overall curvature)." 
%Please note that the first paragraph of a section or subsection is
%not indented. The first paragraph that follows a table, figure,
%equation etc. does not need an indent, either.
